User Study: Comparison of Picture Passwords and Current Login Approaches

In this research, we conduct a user study that compares different computer/system authentication methods. More specifically, we look into comparing regular password authentication with picture authentication. Picture authentication means selecting a sequence of pictures from a set of pictures (30). We present users with both interfaces; various metrics are tracked while the participants conduct a variety of user authentication-related tasks. Other metrics include user perception of security with such technologies.

==> bios.tex <==
\newpage
\section*{About the Authors}
  \vspace{20px}\par

 \begin{wrapfigure}{l}{25mm} 
    % \includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{example-image}
    \includegraphics[width=0.8in,clip,keepaspectratio]{bio-pics/ignacio Cropped (1).jpg}
\end{wrapfigure}\par\
  % \vspace{5px}

  \textbf{Ignacio Astaburuaga} is a Ph.D. student in the Department of Computer Science and Engineering at the University of Nevada, Reno. His research interests include cybersecurity, Quantum, hardware security, and machine learning. He graduated with his B.S in 2019 and M.S. in 2022 from the University of Nevada, Reno, in Computer Science and Engineering.\par
  \vspace{30px}

   \begin{wrapfigure}{l}{25mm} 
    \includegraphics[width=0.8in,clip,keepaspectratio]{bio-pics/SergiuDascalu.jpg}
  \end{wrapfigure}\par
  \textbf{Sergiu Dascalu} is a Professor in the Department of Computer Science and Engineering at the University of Nevada, Reno, which he joined in 2002. He received a Master's degree in Automatic Control and Computers from the Polytechnic University of Bucharest, Romania, and a PhD in Computer Science from Dalhousie University, Halifax, NS, Canada. His main research interests are in the areas of software engineering and human-computer interaction. Sergiu has published over 140 peer-reviewed papers and has been involved in leadership roles in projects funded by industrial companies as well as federal agencies such as NSF, NASA, and ONR. He has advised many PhD and Master's students and is the recipient of several awards and recognitions, including the 2011 UNR Donald Tibbitts Distinguished Teacher of Year award.\par
  \vspace{25px}
